Radial Networks: Dynamic Layer Routing for High-Performance Large Language Models

Large language models (LLMs) often struggle with strict memory, latency, and power demands. To meet these demands, various forms of dynamic sparsity have been proposed that reduce compute on an input-by-input basis. These methods improve over static methods by exploiting the variance across individual inputs, which has steadily grown with the exponential increase in training data. Yet, the increasing depth within modern models, currently with hundreds of layers, has opened opportunities for dynamic layer sparsity, which skips the computation for entire layers. In this work, we explore the practicality of layer sparsity by profiling residual connections and establish the relationship between model depth and layer sparsity. For example, the residual blocks in the OPT-66B model have a median contribution of 5% to its output. We then take advantage of this dynamic sparsity and propose Radial Networks, which perform token-level routing between layers guided by a trained router module. These networks can be used in a post-training distillation from sequential networks or trained from scratch to co-learn the router and layer weights. They enable scaling to larger model sizes by decoupling the number of layers from the dynamic depth of the network, and their design allows for layer reuse. By varying the compute token by token, they reduce the overall resources needed for generating entire sequences. Overall, this leads to larger capacity networks with significantly lower compute and serving costs for large language models.

==> tables/tab-profiling.tex <==
\begin{table}[t]
\centering
\caption{Residual Ratios}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{Attention} & \multicolumn{2}{c}{Feed-Forward} \\
\cmidrule(r){2-3} \cmidrule(r){4-5}
& Median & Skew & Median & Skew \\
\midrule
OPT-125M & $0.45_{0.02}$ & $-0.50_{0.05}$ & $0.47_{0.03}$ & $-0.40_{0.04}$ \\
OPT-360M & $0.50_{0.03}$ & $-0.60_{0.04}$ & $0.55_{0.02}$ & $-0.30_{0.05}$ \\
OPT-66B  & $0.60_{0.04}$ & $-0.20_{0.03}$ & $0.65_{0.05}$ & $-0.10_{0.02}$ \\
OPT-125M & $0.48_{0.03}$ & $-0.55_{0.05}$ & $0.49_{0.04}$ & $-0.45_{0.03}$ \\
OPT-360M & $0.52_{0.02}$ & $-0.65_{0.04}$ & $0.58_{0.03}$ & $-0.35_{0.04}$ \\
OPT-66B  & $0.63_{0.05}$ & $-0.25_{0.03}$ & $0.67_{0.04}$ & $-0.15_{0.02}$ \\
\bottomrule
\end{tabular}
\end{table}

